Convex Geometric Motion Planning on Lie Groups via Moment Relaxation

This paper reports a novel result: with proper robot models on matrix Lie groups, one can formulate the kinodynamic motion planning problem for rigid body systems as \emph{exact} polynomial optimization problems that can be relaxed as semidefinite programming (SDP). Due to the nonlinear rigid body dynamics, the motion planning problem for rigid body systems is nonconvex. Existing global optimization-based methods do not properly deal with the configuration space of the 3D rigid body; thus, they do not scale well to long-horizon planning problems. We use Lie groups as the configuration space in our formulation and apply the variational integrator to formulate the forced rigid body systems as quadratic polynomials. Then we leverage Lasserre's hierarchy to obtain the globally optimal solution via SDP. By constructing the motion planning problem in a sparse manner, the results show that the proposed algorithm has \emph{linear} complexity with respect to the planning horizon. This paper demonstrates the proposed method can provide rank-one optimal solutions at relaxation order two for most of the testing cases of 1) 3D drone landing using the full dynamics model and 2) inverse kinematics for serial manipulators.

==> bak <==
% \begin{problem}[\ref{prob:pocp} as a POP]
% Find the set of optimal state $x_k \in \mathbb{R}^n$ and optimal input $u_k \in \mathbb{R}^m$:
% \begin{equation}
%     \begin{aligned}
%     \label{prob:pop-n}
%     \min_{\mathcal{U_N}} \quad & \Psi(x_{N}) + \sum_{k=0}^{N-1} L(x_k, u_k) \\
%     \text{s.t. } 
%     &\phi(x_0, x(0) \ge 0, \\
%     & g(x_{k+1}, x_k, u_k) \ge 0, \\
%     &k=0,1,\dots,N-1.
%     \end{aligned}% \tag{$\mathbb{P}_N$}
% \end{equation}
% \end{problem}
% Note that any equality constraints could be written as two inequality constraints. Thus we could use $g$ to contain the constraints defined by $F$ and $C$, and we also overload the $\phi$ to denote the initial constrains defined in \eqref{prob:pop-n}. 

% In the next few sections, we use \ref{prob:pop-n} in the context of optimal control and \ref{prob:pocp} in the context of optimization, while we keep in mind that they are equivalent. 


Note that the system dynamics $F$ only link two consecutive step, and the constraints only consider states within a single step, thus \ref{prob:pocp} satisfies the Markov assumption. Therefore, we could use the DP to derive the optimality condition. We define the value function or cost-to-go of $\mathbb{P}_{N}(\bar{x}_0)$ by the recursion:
\begin{equation}
\label{eq:value_fun}
\begin{aligned}
    V_k^{N}(x_k)&:=\min_{\mathcal{U}_{k}^{N}} \Psi(x_{N}) + \sum_{j=k}^{N-1} L(x_j, u_j), \\
    s.t \quad &\phi(x_k, x(k)) = 0 \\
    & F(x_{j+1}, x_{j}, u_j) = 0 \\
    & C(x{j}, u_j) \ge 0 \\
    &j=k,k+1,\dots,N-1.
\end{aligned}
\end{equation}
with $V^N_N(x_N):=\Psi(x_N)$. 

\begin{problem}[One-step Fixed-End POCP]
Given the optimal solution of $\mathbb{P}_N(\bar{x}_0)$, i.e. $\mathcal{U}_N^*$, 
find the set of optimal state $x_0, x_1 \in \mathbb{R}^n$ and optimal input $u_0 \in \mathbb{R}^m$ for
\begin{equation}
    \begin{aligned}
    \label{prob:ofe-pocp}
    \min_{\{x_0, x_1 | u_0\}} \quad &L(x_0, u_0) \\
    \text{s.t. } 
    &\phi(x_0, \bar{x}_0) = 0,\text{  }\phi(x_1, x_1^*) = 0 \\
    & F(x_{1}, x_{0}, u_k) = 0 \\
    & C(x_{0}, u_0) \ge 0 \\
    \end{aligned}\tag{OFE-POCP}
\end{equation}
\end{problem}


% Given a $s(2m)$-sequence $y=(y_{\alpha})$, and let $M_m(y)$ be the moment matrix of dimension $s(m)$, we could construct 

% where we have $x^{\alpha}:=x_1^{\alpha_1}x_2^{\alpha_2}\dots x_n^{\alpha_n},\alpha_i \in \mathbb{N} $ and $\|\alpha\|_1\le m$. We call $x^{\alpha}$ monomial and the $p = \{p_{\alpha}\} \in \mathbb{R}^{s(m)}$ is the coefficients vector. 

% Then, we could define the basis as the set:
% \begin{equation}
%     [x]_{m}:=\{x^{\alpha} | \|\alpha\|_1\le m, \alpha \in \mathbb{Z}^n_{+} \}, 
% \end{equation}


Then we could formulate the moment matrix $M_{m}(x)$:
\begin{equation}
    M_{m}(x):=v_m(x) v_m(x)^{\transpose}
\end{equation}
For example, when $m=2, n=2$, we have the moment matrix $M_2(x)$ as:
\begin{equation}
\begin{aligned}
    {M}_{2}(x) &=[x]_2[x]_2^{\top} \\
    &=\left[\begin{array}{cccccc}
1 & x_1 & x_2 & x_1^2 & x_1 x_2 & x_2^2 \\
x_1 & x_1^2 & x_1 x_2 & x_1^3 & x_1^2 x_2 & x_1 x_2^2 \\
x_2 & x_1 x_2 & x_2^2 & x_1^2 x_2 & x_1 x_2^2 & x_2^3 \\
x_1^2 & x_1^3 & x_1^2 x_2 & x_1^4 & x_1^3 x_2 & x_1^2 x_2^2 \\
x_1 x_2 & x_1^2 x_2 & x_1 x_2^2 & x_1^3 x_2 & x_1^2 x_2^2 & x_1 x_2^3 \\
x_2^2 & x_1 x_2^2 & x_2^3 & x_1^2 x_2^2 & x_1 x_2^3 & x_2^4
\end{array}\right]
\end{aligned}
\end{equation}
We find that the unique entries of in $M_m(x)$ appears in the basis $v_{2m}(x)$, and several entries appear multiple times. 

% \begin{equation}
% \begin{aligned}
%     {M}_{2}(x) &=[x]_2[x]_2^{\top} \\
%     &=\left[\begin{array}{cccccc}
% 1 & x_1 & x_2 & x_1^2 & x_1 x_2 & x_2^2 \\
% x_1 & x_1^2 & x_1 x_2 & x_1^3 & x_1^2 x_2 & x_1 x_2^2 \\
% x_2 & x_1 x_2 & x_2^2 & x_1^2 x_2 & x_1 x_2^2 & x_2^3 \\
% x_1^2 & x_1^3 & x_1^2 x_2 & x_1^4 & x_1^3 x_2 & x_1^2 x_2^2 \\
% x_1 x_2 & x_1^2 x_2 & x_1 x_2^2 & x_1^3 x_2 & x_1^2 x_2^2 & x_1 x_2^3 \\
% x_2^2 & x_1 x_2^2 & x_2^3 & x_1^2 x_2^2 & x_1 x_2^3 & x_2^4
% \end{array}\right]
% \end{aligned}
% \end{equation}

% where we have $x^{\alpha}:=x_1^{\alpha_1}x_2^{\alpha_2}\dots x_n^{\alpha_n},\alpha_i \in \mathbb{N} $ and $\|\alpha\|_1\le m$. We call $x^{\alpha}$ monomial and the $p = \{p_{\alpha}\} \in \mathbb{R}^{s(m)}$ is the coefficients vector. 

% Then, we could define the basis as the set:
% \begin{equation}
%     [x]_{m}:=\{x^{\alpha} | \|\alpha\|_1\le m, \alpha \in \mathbb{Z}^n_{+} \}, 
% \end{equation}


% Then we could formulate the moment matrix $M_{m}(x)$:
% \begin{equation}
%     M_{m}(x):=v_m(x) v_m(x)^{\transpose}
% \end{equation}
% For example, when $m=2, n=2$, we have the moment matrix $M_2(x)$ as:
% \begin{equation}
% \begin{aligned}
%     {M}_{2}(x) &=[x]_2[x]_2^{\top} \\
%     &=\left[\begin{array}{cccccc}
% 1 & x_1 & x_2 & x_1^2 & x_1 x_2 & x_2^2 \\
% x_1 & x_1^2 & x_1 x_2 & x_1^3 & x_1^2 x_2 & x_1 x_2^2 \\
% x_2 & x_1 x_2 & x_2^2 & x_1^2 x_2 & x_1 x_2^2 & x_2^3 \\
% x_1^2 & x_1^3 & x_1^2 x_2 & x_1^4 & x_1^3 x_2 & x_1^2 x_2^2 \\
% x_1 x_2 & x_1^2 x_2 & x_1 x_2^2 & x_1^3 x_2 & x_1^2 x_2^2 & x_1 x_2^3 \\
% x_2^2 & x_1 x_2^2 & x_2^3 & x_1^2 x_2^2 & x_1 x_2^3 & x_2^4
% \end{array}\right]
% \end{aligned}
% \end{equation}
% We find that the unique entries of in $M_m(x)$ appears in the basis $v_{2m}(x)$, and several entries appear multiple times. 


% \tsl{We need to decide whether to introduce the localizing matrix. We need a brief and reader-friendly introduction.}

% $\mathbb{P}_{N-1}$ is tight at order $\kappa$ for generic initial condition $\bar{x}_0$. We now show that the moment relaxation of $\mathbb{P}_{N}$ is also tight at $\kappa$ given that the moment relaxation of \ref{prob:ofe-pocp} is also tight at $\kappa$, for generic initial condition $\bar{x}_0$. 

% By Proposition \ref{prop:t-pocp=pocp}, \ref{prob:t-pocp} and \ref{prob:pocp} are equivalent in the sense that they have the same solution and optimal value. Thus if suffices to analyze the \ref{prob:t-pocp}. By Lemma \ref{lemma:separation}, solving the \ref{prob:t-pocp} is equivalent to solve \ref{prob:ofe-pocp} and $\mathbb{P}_{N-1}(x_1^*)$. By the induction, we have assumed that the moment relaxation of $\mathbb{P}_{N-1}(x_1^*)$ is tight at order $\kappa$. We also assume that the moment relaxation \ref{prob:ofe-pocp} is also tight at $\kappa$. 

% The next step is to show that the tight relaxation of $\mathbb{P}_{N-1}(x_1^*)$ and \ref{prob:ofe-pocp} will characterize another tight relaxation of $\mathbb{P}_N(\bar{x})$. 

% If the moment relaxation of $\mathbb{P}_{N-1}(x_1^*)$ and \ref{prob:ofe-pocp} are tight, we have that:
% \begin{equation}
%     \mathbb{P}_{N-1}(x_1^*) = SOS + f^*
% \end{equation}
% and 
% \begin{equation}
%     OFE-POCP = SOS + f^*
% \end{equation}
% Sum them up, we have the result. 

% \tsl{We only need to show that the T-POCP have the form of the tight relaxation.}

% \tsl{IMPORTANT!!! When we add things up, we can delete the constraints realted to the equality constraints and the other stuff has the exact construction of the optimality condition. }
% Note that the $V_(x_k)$ could be derived by another $\mathbb{P}_{N-1}$ with initial $x_k$. Now we suppose that the optimal control problem 

% For the $\mathbb{P}_{N}$, we apply the DP to convert it to the optimization problem in \eqref{eq:q_fun}. 


#########################################################
################# Constrained LGVI ######################
#########################################################
\subsection{Continuous-time Lagrangian dynamics}
% \tsl{Need a remark about the non-holonomic constraints.} 
Consider a mechanical system evolving on the configuration manifold $Q$. Then the velocity evolves on the tangent space $TQ$.  We denote the configuration state as $q \in Q$ and the generalized velocity as $\dot{q} \in T_{q}Q$. Then the Lagrangian is a map $L:TQ\rightarrow \mathbb{R}$. 

Consider the kinetic energy $T(\dot{q})$, potential energy $V(q)$, a $m$ dimensional holonomic constraints $g(q) = 0  \in \mathbb{R}^m$ and the corresponding constrained force $\lambda \in \mathbb{R}^m$. Thus we have an constrain manifold $C=\{q|q\in Q, g(q) = 0\}$. Then we could obtain the Lagrangian 

\begin{equation}
\label{eq:ct_lag}
    \bar{L}(q, \dot{q}, \lambda) = L(q, \dot{q}) - g(q)^{\transpose}\lambda,
\end{equation}
with the unconstrained part defined by 
\begin{equation}
    L(q, \dot{q}):=T(\dot{q}) - V(q). 
\end{equation}
For the forced system, we consider the external force $f\in \mathbb{R}^r$ and an input influence map $B: \mathbb{R}^r \rightarrow \mathbb{R}^n$. Given such an external force, we seek the stationary point of the action according to the Lagrange-d'Alambert principle; thus we have:
\begin{equation}
    \delta \left( \int_0^T\bar{L}(q, \dot{q})dt -\int_0^{T}Bf(t)\cdot\delta q dt \right)=0 ,
\end{equation}
where $\delta$ denotes the variation vanishing at the endpoints. Using the integration by part, we have the Euler-Lagrange equations for the forced and constrained system:
\begin{equation}
\label{eq:ct_eom}
\begin{aligned}
    \frac{d}{dt}\left( \frac{\partial L(q, \dot{q})}{\partial \dot{q}} \right) - \frac{\partial L(q, \dot{q})}{\partial q} + G(q)^{\transpose} \lambda = f \\
    g(q) = 0 ,
\end{aligned}
\end{equation}
where $G := \frac{\partial g}{\partial q}$ and the term $G(q)^{\transpose}\lambda \perp T_qC$ ensures that the configuration states do not leave the constrained manifold $C$. 

% Corresponding constrained Euler-Lagrange equations:
% \begin{equation}
% \begin{aligned}
%     \frac{d}{dt}\left( \frac{\partial L(q, \dot{q})}{\partial \dot{q}} \right) - \frac{\partial L(q, \dot{q})}{\partial q} + G(q)^{\transpose} \lambda = 0 \\
%     g(q) = 0 
% \end{aligned}
% \end{equation}
% $\lambda \in \mathbb{R}^m$ the constrained force and $G := \frac{\partial g}{\partial q}$.

#######################################################
############### INTRODUCTIO ###########################
#######################################################


% The recent concepts of certifiable algorithm \cite{bandeira2016note} have been applied in robot perception problems \cite{yang2022certifiably, rosen2019se, fan2020cpl}. As is summarized by \cite{yang2022certifiably} and \cite{bandeira2016note}, a certifiable algorithm requires that: (i) the algorithm runs in polynomial time, (ii) returns a globally optimal solution with a certificate of the optimality, (iii) or fails to do so but provide a bound on the objective value. When the relaxation order of Lasserre's hierarchy is determined, the SDP in fixed size can be solved in polynomial time. The optimum of SDP can also be certified via rank conditions of the moment matrix or serve as a lower bound estimation for the problem \cite{lasserre2015introduction}. Such properties are seldom seen in the existing motion planning algorithms based on sampling, combinatorial solvers, or nonlinear local solvers. 

% The primal SDP relaxation of Lasserre's hierarchy could be interpreted as a general moment problem that tries to find a moment matrix that minimize a infinite dimensional linear programming. While the dual of the primal SDP relaxation is to find a set of SOS certificate that certify the global optimality. 

\tsl{I deleted the integrator part.}
% As these methods only consider the $SO(2)$ rotational group for revolute joints, the order of monomials involved will grow linearly with the length of the kinematic chain % For series manipulator of 7 degree of freedom, these methods are tractable.  

% For motion planning from dynamic level, converting the configuration space to polynomial via Taylor expansion or approximating by intervals would not scale good for high accuracy and long horizon methods.
% All the reviewed methods applies the trivial or simplified models, while omitted the actual dynamics. To the best of the author's knowledge, there is not an effective global optimal formulation for dynamic level planning. 

% TODO: planning paper with trivial dynamics. 
% el2021piecewise
% Ashkan paper, Lasserre
% The key insight of this work is to approximate the nonlinear term (sin/cos) via piece-wise linear functions, thus 

% \subsubsection{Geometric robot formulation}
% The equations of motion of a multi-body robot can be obtained by Euler-Lagrange equation \cite{bloch2003nonholonomic, marsden1998introduction}. 
% Most trajectory optimization methods use minimal coordinates, such as joint angles, to describe the robot dynamics. Therefore, the integration scheme such as explicit Euler~\cite{posa2014direct, hereid2017frost} can be applied for the vector field dynamics as no explicit constraints are needed. % However, the minimal coordinates increases the nonlinearities in the robot model by introducing high order trigonometric term. With minimal coordinates, each degree of freedom is represented by one parameter. Thus, there is no need to model the constraints between each rigid body explicitly.

% Another promising way of representing the dynamics is the maximal coordinates, where six degrees of freedom of each rigid body is modeled, along with explicit constraints between them \cite{brudigam2021integrator, brudigam2021LQR}. 
% % Consider that the dynamics of each rigid body could be described by the Euler Poincare equation \cite{marsden1998introduction, bloch2003nonholonomic} on matrix Lie groups, which is a set of second-order polynomial, the maximal coordinates formulation has great potential in the low-order polynomial formulations for general robotics model. 
% As the Lie group formulation models the rigid body on manifolds, the integration scheme is not as intuitive as in vector space. The simplest explicit (Lie-) Euler integration for rigid body dynamics on $SE(3)$ results in an exponential map, making it challenging to be represented by polynomials with finite order \cite{celledoni2014introduction, iserles2000lie}. The reason is that the conventional integrator discretizes the continuous time equation of motion and, therefore, has to lift the integration from tangent space to the manifold. While the variational integrator solves the problem by using the configuration states to represent the velocities  and then discretize the Lagrangian \cite{marsden2001discrete}. The research \cite{brudigam2021integrator} applied the quaternion-based variational integrator in maximal coordinates for robot numerical simulations. Though quaternion has the smallest number of parameters to describe rotation while avoiding singularities, the resulting equations still involve root square term. The Lie group variational integrator (LGVI) solves the problem by directly using the matrix Lie group as the configuration manifold. As such, one can obtain a robot model in completely quadratic polynomial form on matrix Lie group~\cite{lee2005lie, lee2007lie, nordkvist2010lie, marsden1999discrete}. 

% As a byproduct, the variational integrator also exhibit superior energy preserving property that.
% \tsl{Several paper from Zach about the application of LGVI. }
% One intuition of the formulation is the increase of dimension decreases the nonlinearity.  Thus, The resulting implicit integrator could fully utilize the property of the configuration space \mgj{what does it mean? I thought variational integrators preserve symmetry (energy, momentum, etc.)}.
% The work \cite{brudigam2021LQR} applied the LQR controller to constrained multi-body system using maximal coordinates. The result suggests that the change of coordinates enables the linear feedback to approximate the nonlinear optimal controller designed in minimal coordinates. 

% Thus, one has to deal with complicated Riemmanian manifolds \cite{bullo1999tracking, bullo2019geometric}, and has to deal with high-order Taylor expansion if applying the SOS relaxations \cite{tedrake2010lqr, majumdar2017funnel}. % To apply the SOS relaxation, applying Taylor expansions would also not scale good for high-order approximation. 

% To apply the POP, the key challenges is to obtain a polynomial robotics model in discrete time. % The generalized velocities are described in the tangent space of the configuration manifold.

% \tsl{The concepts of certifiable optimality is proposed by SOS people. }
% The first-order methods. The first order based trajectory optimization methods has gain huge success in the past decades. Hard to certify the global optimality? 

% The implicit integrator. 

% general moment problem


#########################################################
################# Lasserre's hierarchy ##################
#########################################################

% The moment matrix \eqref{eq:moment_matrix} defines a bilinear form, such that:
% \begin{equation}
% \begin{aligned}
%      \langle p, q \rangle_y &:= L_y(pq) = \langle p, M_m(y) q \rangle \\
%     &= p^{\transpose}M_m(y)q, \quad \forall p, q \in \mathbb{R}^{s(m)}. 
% \end{aligned}
% \end{equation}
Given a polynomial $u\in\mathbb{R}[x]$ with coefficient $u = \{u_{\gamma}\}$, Then we could define the \emph{localizing matrix} for $u$ and $y$ as:
\begin{equation}
\begin{aligned}
    M_m(uy)(\alpha, \beta) &= \mathcal{L}_y(u(x)x^{\alpha} x^{\beta})\\
    &= \sum_{\gamma} u_{\gamma}y_{\gamma+\alpha + \beta}, \alpha, \beta \in \mathbb{N}_r^n.
\end{aligned} 
\end{equation}
 Similarly, we have the equivalent definition 
 \begin{equation}
    M_m(uy) = \mathcal{L}_y(uv_r(x)v_r(x)^{\transpose}).
\end{equation}

Now we introduce several key concepts for the moment matrix. Suppose $y = (y_{\alpha}) \subset \mathbb{R}$ be an sequence indexed by 
$\alpha \in \mathbb{N}_r^n$, and let the $\mathcal{L}_y: \mathbb{R}[x] \rightarrow \mathbb{R}$ be the linear functional:
\begin{equation}
\label{eq:functional}
    f(x) = \sum_{\alpha} f_{\alpha} x^{\alpha} \mapsto \mathcal{L}_y(f) = \sum_{\alpha} f_{\alpha}y_{\alpha}. % \mathbb{N}^{m}
\end{equation}
The functional \eqref{eq:functional} can be interpreted as substituting the monomials $x^{\alpha}$ in $f(x)$ by $y_\alpha$ with the same index $\alpha$ to obtain the numerical value. % For the general moment problem, our goal would be to find such an moment sequence $y_{\alpha}$ that admit a representing measure. 

Given a $s(2r)$-sequence $y=(y_{\alpha})$, let $M_r(y)$ be the moment matrix of dimension $s(r) \times s(r)$, with rows and columns labeled the same as in \eqref{eq:basis}. Then the moment matrix can be constructed by:
\begin{equation}
\label{eq:moment_matrix}
    M_m(y)(\alpha, \beta) = \mathcal{L}_y(x^{\alpha} x^{\beta}) = y_{\alpha + \beta}, \alpha, \beta \in \mathbb{N}_r^n. 
\end{equation}
Or equivalently, we can manipulate a whole matrix entry-wise:
\begin{equation}
    M_m(y) = \mathcal{L}_y(v_r(x)v_r(x)^{\transpose}). 
\end{equation}
Note that the element in $y\in \mathbb{R}^{s(2r)}$ may appear multiple times in the moment matrix.

% \begin{problem}[Infinite dimension linear programming]
% \begin{equation}
% \label{prob:inf-lp}
% \begin{aligned}
%     p^*&:=\min_{\mu\in\mathcal{M}^+(\mathbb{K})} \int_{\mathbb{K}} p(x) d\mu \\
% \end{aligned}\tag{LP}
% \end{equation}
% with $\mathbb{K}$ the feasible set defined in \eqref{prob:pop}, $\mathcal{M}(\mathbb{K})$ the set of vector space of finite signed Borel measure and $\mathcal{M}^+(\mathbb{K})$ the convex cone of nonnegative finite Borel measure on $\mathbb{K}$. 
% \end{problem}
% Therefore, the optimization problem \eqref{prob:pop} is equivalent to finding the Dirac measure $\delta_{x^*}$ that is associated with the minimizer $x^*$ of \eqref{prob:pop}. Recall that the Dirac measure has the property: $$\int_{\mathbb{K}} p(x) d \delta_{\bar{x}} = p(\bar{x}), $$
% that enable one to select the value of $p(x)$ at given point $\bar{x}$.

% As $p(x)$ is a polynomial, the objective function $\int_{\mathbb{K}} p(x) d\mu$ would be a linear combination of the terms that appeared in the moment matrix associated with the measure $\mu$. Therefore, one can search over the moment sequence $y_{\alpha}$ (infinite) and verify that $y_{\alpha}$ is a moment sequence of a measure with support contained in $\mathbb{K}$. This verifying process is the $\mathbb{K}$-moment problem \cite{lasserre2015introduction}. % that checking the sequence $y$ are moment sequence of a measure with support in $\mathbb{K}$. 

% truncated $\mathbb{K}$-moment problem:
% When the problem \eqref{prob:pop_sdp} is solved, one could check the following rank condition to verify if the minimizer indeed admits a representing measure:  % \tsl{Introduce the representing measure somewhere? }
\begin{theorem}[Sufficient condition for truncated $\mathbb{K}$-moment problem \cite{lasserre2015introduction} ]
    Let $\mathbb{K}$ be the feasible set defined by polynomial $g_i$ and $h_i$ defined in \eqref{prob:pop}. Then the moment sequence $y_{\alpha}$ has a $\operatorname{rank}(M_{\kappa-d_g})$-atomic representing measure $\mu$ with support contained in $\mathbb{K}$ if and only if:
    \begin{enumerate}
        \item $M_{\kappa}(y) \ge 0$, $M_{\kappa - d_g}(g_jy) \ge 0$, $j = 1, 2, \dots, m$, and, 
        \item $M_{\kappa}(y) = M_{\kappa - d_g}(y)$. 
    \end{enumerate}
\end{theorem}

##################################################################
####################        LGVI       ###########################
##################################################################
\section{Variational Integrator}

In this section, we introduce the discrete Lagrangian dynamics via the variational integrator. % We show that the rigid body system can be represented by polynomial dynamics with quadratic constraints.  

\subsection{Continuous-time Lagrangian dynamics}
% \tsl{Need a remark about the non-holonomic constraints.} 
Consider a mechanical system evolving on the configuration manifold $Q$. We have the configuration state as $q \in Q$ and the generalized velocity as $\dot{q} \in T_{q}Q$. Consider the kinetic energy $T(\dot{q})$, potential energy $V(q)$. Then we have the Lagrangian:
\begin{equation}
\label{eq:ct_lag}
    L(q, \dot{q}):=T(\dot{q}) - V(q). 
\end{equation}
For the forced system, we consider the external force $f\in \mathbb{R}^r$ and an input influence map $B: \mathbb{R}^r \rightarrow \mathbb{R}^n$. Given such an external force, we seek the stationary point of the action according to the Lagrange-d'Alambert principle; thus we have:
\begin{equation}
    \delta \left( \int_0^T{L}(q, \dot{q})dt -\int_0^{T}Bf(t)\cdot\delta q dt \right)=0 ,
\end{equation}
where $\delta$ denotes the variation vanishing at the endpoints. Using the integration by part, we have the Euler-Lagrange equations for the forced and constrained system:
\begin{equation}
\label{eq:ct_eom}
\begin{aligned}
    \frac{d}{dt}\left( \frac{\partial L(q, \dot{q})}{\partial \dot{q}} \right) - \frac{\partial L(q, \dot{q})}{\partial q} = f. \\
\end{aligned}
\end{equation}

% Corresponding constrained Euler-Lagrange equations:
% \begin{equation}
% \begin{aligned}
%     \frac{d}{dt}\left( \frac{\partial L(q, \dot{q})}{\partial \dot{q}} \right) - \frac{\partial L(q, \dot{q})}{\partial q} + G(q)^{\transpose} \lambda = 0 \\
%     g(q) = 0 
% \end{aligned}
% \end{equation}
% $\lambda \in \mathbb{R}^m$ the constrained force and $G := \frac{\partial g}{\partial q}$.

\subsection{Discrete-time Lagrangian dynamics}
 % The discrete Lagrangian is defined as a function $L_d:Q\times Q \rightarrow \mathbb{R}$. 


% For the same configuration state $Q$, the discrete state space is defined as $Q\times Q$. We then introduce a time step $h \in \mathbb{R}$. Then discrete Lagrangian $L_d: Q\times Q \rightarrow \mathbb{R}$ is  that represents the velocity between via configuration state $q\in Q$ in consecutive time step.  Thus the discrete Lagrangian $L_d: Q\times Q \rightarrow \mathbb{R}$ could be considered as the approximation of the action integral via: 
The key idea of a variational integrator is to discretize the Lagrangian \eqref{eq:ct_lag} instead of the equation of motion \eqref{eq:ct_eom}. The discretization scheme ensures that the Lagrangian is conserved in the discrete-time, thus having superior energy conservation in the long duration. 

For the same configuration state $Q$, we define discrete state space as $Q\times Q$ that relates the states in the consecutive time step. We then introduce the time step $h \in \mathbb{R}$ and the time sequence $\{t_k = kh | k = 0, \dots, N\} \subset \mathbb{R}$. Thus the discrete Lagrangian $L_d: Q\times Q \rightarrow \mathbb{R}$ could be considered as the approximation of the action integral via:

\begin{equation}
    L_d(q_k, q_{k+1}) \approx \int ^{t_{k+1}}_{t_k}L(q, \dot{q})dt
\end{equation}
In this work, we consider the midpoint approximation:
\begin{equation}
\label{eq:dt_lag_int}
    L_d(q_k, q_{k+1}) = hT(\frac{q_{k+1} - q_k}{h}) - hV(\frac{q_{k+1} + q_k}{2}),
\end{equation}
% Note that in this step, the generalized velocity $\dot{q}$ is approximated by $q$, thus one can fully utilize the structure of $q$. 
% Similarly, the integration of the constraints could be approximated as:
% \begin{equation}
% \label{eq:dt_cons_int}
%     \int_{t_k}^{t_{k+1}}-g^{\transpose}\lambda \approx -\frac{1}{2}g_d(q_k)^{\transpose}\lambda_k - \frac{1}{2}g_d(q_{k+1})^{\transpose}\lambda_{k+1}
% \end{equation}
Similarly, the integration of the external force could be approximated as:
\begin{equation}
\label{eq:dt_force_int}
    \int_{t_k}^{t_{k+1}}-Bf(t)\cdot\delta q \approx -\frac{1}{2}Bf_d(t_k)\cdot \delta q_{k} - \frac{1}{2} Bf_d(t_{k+1})\cdot \delta q_{k+1}.
\end{equation}
% where $g_d(q_k):=hg(q_k)$ and $f_d(t_k) := hf(t_k)$. 

Then the discrete variant of the action integration becomes:
\begin{equation}
    S_d = \sum_{k=0}^{N-1}{L}_d(q_k, q_{k+1}),  
\end{equation}
where $\bar{L}_d(q_k, q_{k+1})$ is the sum of the midpoint approximation defined in \eqref{eq:dt_lag_int} and \eqref{eq:dt_force_int}. Finally, we group the term corresponding to $\delta q_{k}$ as the discrete version of integration by part \cite{marsden2001discrete}: 
\begin{equation}
\begin{aligned}
  \delta S_d &= D_1 \bar{L}_d(q_0, q_1) \cdot \delta q_0 +  D_2 \bar{L}_d(q_{k-1}, q_k) \cdot \delta q_N\\ 
    &+ \sum_{k=1}^{N-1}
    \left( D_2 \bar{L}_d(q_{k-1}, q_k) + D_1 \bar{L}_d(q_k, q_{k+1})\right) \cdot \delta q_k. 
\end{aligned}
\end{equation}
where $D_i$ denotes the derivative with respect to the $i_{th}$ argument. 
By the least action principle, the stationary point could be derived: 
\begin{equation}
\begin{aligned}
D_1L_d(q_k, q_{k+1}) + D_2L_d(q_{k-1}, q_{k}) =Bf_d(t_k)
\end{aligned}
\end{equation}
% and $\delta q_0 = \delta q_N = 0$ as they vanish at the end point.

% For now, we could the discrete variant of the Lagrangian dynamics when we specify the configuration states, kinetic energy and the constraints. 
% The integral of the constraints and constrained force can be approximated by:
% \begin{equation}
%     \frac{h}{2}\left( g^{\transpose}(q_n)\lambda_n + g^{\transpose}(q_{n+1})\lambda_{n+1}\right) \approx \int_{t_n}^{t_{n+1}} g^{\transpose}\lambda dt
% \end{equation}
% Thus we have the discrete Euler Lagrangian equations:
% \begin{equation}
% \begin{aligned}
%   D_1L_d(q_n, q_{n+1}) + D_2L_d(q_{n-1}, q_{n}) + G_d^{\transpose}(q_n)\lambda_n = 0,\\
%     g(q_{n+1}) = 0
% \end{aligned}
% \end{equation}

% % Note that take the variation in the tangent space $\mathfrak{se}(3)$. 
% \subsection{LGVI for multi-body}
% Based on the dynamics of SRB, we could derive the dynamics for multi-body system. Similarly, we here choose the configuration space as $q \in \left(SE(3)\times SE(3) \times \cdots  \times SE(3) \right)$, and we consider the constraints between SRB $i$ and $j$ as $g_{ij}(q)$
% For holonomic constraints like joints or contact, we have $g$ only contain element up to two degree. Thus we have the dynamics of the following form:
% \begin{equation}
% \begin{aligned}
%     &\frac{1}{h}(F^i_{k+1}I_b^i - I_b^iF^i_{k} - I_b^iF_{k+1}^{i\transpose} + F_k^{i\transpose}I_b^i) + h\tau^i_k + \Sigma hG^{ij\transpose}_k\lambda^{ij}_k = 0 \\
%     &m_iv^i_{k+1} = m_iv^i_{k} + h^2u^i_k + h^2R_{k+1}U + \Sigma h^2G^{ij\transpose}_k\lambda^{ij}_k\\
%     &R^i_{k+1} = R^i_kF^i_k, \ \ \ p^i_{k+1} = hR^i_kv^i_k + p^i_k \\
%     &g^{ij}(X^i_{k+1}, X^j_{k+1}) = 0
% \end{aligned}
% \end{equation}
% where $g_{ij}$ is the constraints between rigid body $i$ and $j$. Note that $i=j$ means the constraints only involve this specific SRB. 


####################################################################
###################  LGVI very simple ##############################
###################################################################

% \tsl{Need a remark about the non-holonomic constraints.} 
Consider a $n$ dimensional mechanical system with the configuration space $Q$, We denote the configuration state as $q \in Q$ and the generalized velocity as $\dot{q} \in T_{q}Q$. Then we have the Lagrangian given the kinetic energy $T(\dot{q})$, potential energy $V(q)$:
\begin{equation}
\label{eq:ct_lag}
    L(q, \dot{q}):=T(\dot{q}) - V(q). 
\end{equation}
The key idea of a variational integrator is to discretize the Lagrangian \eqref{eq:ct_lag} to obtain the discrete equation of motion. The discretization scheme ensures that the Lagrangian is conserved in the discrete-time, thus having superior energy conservation in the long duration. 

We define the time step $h \in \mathbb{R}$ and the time sequence $\{t_k = kh | k = 0, \dots, N\} \subset \mathbb{R}$. Thus the discrete Lagrangian $L_d: Q\times Q \rightarrow \mathbb{R}$ could be considered as the approximation of the action integral via:

\begin{equation}
    L_d(q_k, q_{k+1}) \approx \int ^{t_{k+1}}_{t_k}L(q, \dot{q})dt
\end{equation}
In this work, we consider the midpoint approximation:
\begin{equation}
\label{eq:dt_lag_int}
    L_d(q_k, q_{k+1}) = hT(\frac{q_{k+1} - q_k}{h}) - hV(\frac{q_{k+1} + q_k}{2}),
\end{equation}
% Similarly, the integration of the external force could be approximated as:
% \begin{equation}
% \label{eq:dt_force_int}
%     \int_{t_k}^{t_{k+1}}-Bf(t)\cdot\delta q \approx -\frac{1}{2}Bf_d(t_k)\cdot \delta q_{k} - \frac{1}{2} Bf_d(t_{k+1})\cdot \delta q_{k+1}.
% \end{equation}
Then the discrete variant of the action integration becomes:
\begin{equation}
    S_d = \sum_{k=0}^{N-1}{L}_d(q_k, q_{k+1}),  
\end{equation}
% where $\bar{L}_d(q_k, q_{k+1})$ is the sum of the midpoint approximation defined in \eqref{eq:dt_lag_int} and \eqref{eq:dt_force_int}. 
Finally, we group the term corresponding to $\delta q_{k}$ as the discrete version of integration by part \cite{marsden2001discrete}: 
\begin{equation}
\begin{aligned}
  \delta S_d &= D_1 \bar{L}_d(q_0, q_1) \cdot \delta q_0 +  D_2 \bar{L}_d(q_{k-1}, q_k) \cdot \delta q_N\\ 
    &+ \sum_{k=1}^{N-1}
    \left( D_2 \bar{L}_d(q_{k-1}, q_k) + D_1 \bar{L}_d(q_k, q_{k+1})\right) \cdot \delta q_k. 
\end{aligned}
\end{equation}
where $D_i$ denotes the derivative with respect to the $i_{th}$ argument. 
By the least action principle, the stationary point could be derived: 
\begin{equation}
\begin{aligned}
D_1L_d(q_k, q_{k+1}) + D_2L_d(q_{k-1}, q_{k}) = 0. % Bf_d(t_k)
\end{aligned}
\end{equation}

